Assessing the Privacy Cost in Centralized Event-Based Demand Response for Microgrids

Demand response (DR) programs have emerged as a potential key enabling ingredient in the context of smart grid (SG). Nevertheless, the rising concerns over privacy issues raised by customers subscribed to these programs constitute a major threat towards their effective deployment and utilization. This has driven extensive research to resolve the hindrance confronted, resulting in a number of methods being proposed for preserving customers' privacy. While these methods provide stringent privacy guarantees, only limited attention has been paid to their computational efficiency and performance quality. Under the paradigm of differential privacy, this paper initiates a systematic empirical study on quantifying the trade-off between privacy and optimality in centralized DR systems for maximizing cumulative customer utility. Aiming to elucidate the factors governing this trade-off, we analyze the cost of privacy in terms of the effect incurred on the objective value of the DR optimization problem when applying the employed privacy-preserving strategy based on Laplace mechanism. The theoretical results derived from the analysis are complemented with empirical findings, corroborated extensively by simulations on a 4-bus MG system with up to thousands of customers. By evaluating the impact of privacy, this pilot study serves DR practitioners when considering the social and economic implications of deploying privacy-preserving DR programs in practice. Moreover, it stimulates further research on exploring more efficient approaches with bounded performance guarantees for optimizing energy procurement of MGs without infringing the privacy of customers on demand side.

==> append.tex <==
\appendix
In the appendix, the full proof of Theorem~\ref{thm} is presented.

\subsection{Proof of Theorem \ref{thm}}

\begin{proof}
	Since $n$ independent samples are drawn from the Laplace distribution the $(\epsilon, \delta)$-differential privacy follows directly from Theorem~\ref{thm2}.
	
	Given that with probability at least $\frac{1-\beta}{n}$, where $\beta \in [0,1]$, the magnitude of a single draw from Laplace distribution with chosen scale parameter is upper bounded by $\frac{\alpha}{2} \triangleq \frac{2u^{\max}\sqrt{8n\log(\frac{n}{\delta})}}{\epsilon}$, then by the union bound this condition holds with probability $1-\beta$ for all $n$ draws.
	
	
	Denote by $x^*$ and $\hat{x}^*$ the optimal solutions of {\sc UMDR$_\textsc{L}$} and {\sc UMPDR$_\textsc{L}$} problems, respectively. Also, let $\Opt_{\textsc{L}}$ be the corresponding total valuation of the optimal solution $x^*$ to {\sc UMDR$_\textsc{L}$}. Note that $\hat{x}^*$ is also a feasible solution to {\sc UMDR$_\textsc{L}$}.
	The additive optimality bound is proved by contradiction. Assume $\sum_{k\in\cN} u_{k,t}\hat{x}^*_k < \Opt_{\textsc{L}} - \alpha$.
	The noise added at time $t\in \cT$ to each customer's utility $u_{k,t}$ is bounded by $\frac{\alpha}{2}$, thus if $\sum_{k\in \cN} u_{k,t}\hat{x}_k^* < \Opt_{\textsc{L}} - \alpha$ then 
	\begin{eqnarray}
	\sum_{k\in\cN}\hat{u}_{k,t}\hat{x}_{k}^* & < &  \sum_{k\in\cN}(u_{k,t}+\frac{\alpha}{2})\hat{x}_{k}^* \\
	& < &\sum_{k\in\cN}u_{k,t}\hat{x}_{k}^* +\sum_{k\in\cN}\frac{\alpha}{2}\hat{x}_{k}^*\\
	& < & \Opt_{\textsc{L}} - \alpha  + \frac{\alpha}{2} \sum_{k\in\cN}\hat{x}_{k}^*\\
	& < & \Opt_{\textsc{L}} - \frac{\alpha}{2} \,. \label{eq2}
	\end{eqnarray}
	The last inequality holds since it is assumed that optimal solution has $l_1$ norm of $1$. Note that one may easily scale down the original perturbed problem {\sc UMPDR$_\textsc{L}$} so as the resulting scaled variant has a solution $\hat{x}^*$ with $l_1$ norm of $1$.
	On the other hand, it follows from the property of the Laplace distribution that
	\begin{eqnarray}
	\sum_{k\in\cN}\hat{u}_{k,t}x_{k}^* &\geq& \sum_{k\in\cN}\Big(u_{k,t}-\frac{\alpha}{2}\Big)x_{k}^* \\
	&\geq &\sum_{k\in\cN}u_{k,t}x_{k}^*  - \frac{\alpha}{2} \\
	&\geq& \Opt_{\textsc{L}} - \frac{\alpha}{2} \, . \label{eq1}
	\end{eqnarray}
	Eqns.~\raf{eq1} and \raf{eq2} together contradict the optimality of $\hat{x}^*$. This completes the proof of the theorem showing that $\sum_{k\in\cN} u_{k,t}\hat{x}^*_k \geq \Opt_{\textsc{L}} - \alpha$.
\end{proof}

\begin{thm}[\cite{5670947}]\label{thm2}
The composition of $n$ adaptively chosen $\epsilon^{\prime}$-differentially private mechanisms is $(\epsilon, \delta)$-differentially private if for $\forall \delta \in (0,1)$ the following holds
$$\epsilon^{\prime} = \frac{\epsilon}{\sqrt{8n\log(\frac{1}{\delta})}}\,.$$
\end{thm}

==> literature.tex <==
\section{Related Work}\label{literature}



==> problem.tex <==
\section{Problem Formulation}\label{problem}
